Splitting a Hybrid ASP Program

Hybrid Answer Set Programming (Hybrid ASP) is an extension of Answer Set Programming (ASP) that allows ASP-like rules to interact with outside sources. The Splitting Set Theorem is an important and extensively used result for ASP. The paper introduces the Splitting Set Theorem for Hybrid ASP, which is for Hybrid ASP the equivalent of the Splitting Set Theorem, and shows how it can be applied to simplify computing answer sets for Hybrid ASP programs most relevant for practical applications.

==> eptcsdata.tex <==
\providecommand{\firstpage}{21}
\providecommand{\publicationstatus}{F. Ricca, A. Russo et al. (Eds.): Proc.\ 36th International Conference \\
on Logic Programming (Technical Communications) 2020 (ICLP 2020)\\
EPTCS 325, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.325.8}{10.4204/EPTCS.325.8}}

